Analysis of functionally graded material plates using triangular elements with cell-based smoothed discrete shear gap method

In this paper, a cell based smoothed finite element method with discrete shear gap technique is employed to study the static bending, free vibration, mechanical and thermal buckling behaviour of functionally graded material (FGM) plates. The plate kinematics is based on the first order shear deformation theory and the shear locking is suppressed by a discrete shear gap method. The shear correction factors are evaluated by employing the energy equivalence principle. The material property is assumed to be temperature dependent and graded only in the thickness direction. The effective properties are computed by using the Mori-Tanaka homogenization method. The accuracy of the present formulation is validated against available solutions. A systematic parametric study is carried out to examine the influence the gradient index, the plate aspect ratio, skewness of the plate and the boundary conditions on the global response of the FGM plates. The effect of a centrally located circular cutout on the global response is also studied.

==> fsdtPlate.tex <==
\subsection{Reissner-Mindlin plate theory} The Reissner-Mindlin plate theory, also known as the first order shear deformation plate theory (FSDT) is an extension of the classical plate theory (or, the Kirchhoff - Love plate theory). The FSDT takes into account the shear deformations through the thickness and are intended for thick plates in which the normal to the medium surface remains straight but not necessarily perpendicular to the medium surface. Using the Mindlin formulation, the displacements $u,v,w$ at a point $(x,y,z)$ in the plate (see \fref{fig:platefig}) from the medium surface are expressed as functions of the mid-plane displacements $u_o,v_o,w_o$ and independent rotations $\theta_x,\theta_y$ of the normal in $yz$ and $xz$ planes, respectively, as

\begin{figure}[htpb]
\centering
\includegraphics[scale=0.6]{./Figures/plate}
\caption{Coordinate system of a rectangular plate.}
\label{fig:platefig}
\end{figure}

\begin{align}
u(x,y,z,t) &= u_o(x,y,t) + z \theta_x(x,y,t) \nonumber \\
v(x,y,z,t) &= v_o(x,y,t) + z \theta_y(x,y,t) \nonumber \\
w(x,y,z,t) &= w_o(x,y,t) 
\label{eqn:displacements}
\end{align}
where $t$ is the time. The strains in terms of mid-plane deformation can be written as:
\begin{equation}
\bveps  = \left\{ \begin{array}{c} \bveps_p \\ \mathbf{0} \end{array} \right \}  + \left\{ \begin{array}{c} z \bveps_b \\ \bveps_s \end{array} \right\} 
\label{eqn:strain1}
\end{equation}
The midplane strains $\bveps_p$, the bending strains $\bveps_b$ and the shear strains $\varepsilon_s$ in \Eref{eqn:strain1} are written as:

\begin{equation}
\renewcommand{\arraystretch}{1.5}
\bveps_p = \left\{ \begin{array}{c} u_{o,x} \\ v_{o,y} \\ u_{o,y}+v_{o,x} \end{array} \right\}, \hspace{1cm}
\renewcommand{\arraystretch}{1.5}
\bveps_b = \left\{ \begin{array}{c} \theta_{x,x} \\ \theta_{y,y} \\ \theta_{x,y}+\theta_{y,x} \end{array} \right\} , \hspace{1cm}
\renewcommand{\arraystretch}{1.5}
\bveps_s = \left\{ \begin{array}{c} \theta _x + w_{o,x} \\ \theta _y + w_{o,y} \end{array} \right\}.
\renewcommand{\arraystretch}{1.5}
\end{equation}
where the subscript `comma' represents the partial derivative with respect to the spatial coordinate succeeding it. The membrane stress resultants $\bn$ and the bending stress resultants $\bm$ can be related to the membrane strains, $\bveps_p$ and the bending strains $\bveps_b$ through the following constitutive relations:

\begin{equation}
\bn = \left\{ \begin{array}{c} N_{xx} \\ N_{yy} \\ N_{xy} \end{array} \right\} = \mathbf{A} \bveps_p + \BB \bveps_b - \bn^\textup{th}, \hspace{0.5cm}
\bm = \left\{ \begin{array}{c} M_{xx} \\ M_{yy} \\ M_{xy} \end{array} \right\} = \BB \bveps_p + \DD \bveps_b - \bm^\textup{th}.
\end{equation}
where the matrices $\mathbf{A} = A_{ij}, \BB= B_{ij}$ and $\DD = D_{ij}; (i,j=1,2,6)$ are the extensional, the bending-extensional coupling and the bending stiffness coefficients and are defined as:

\begin{equation}
\left\{ A_{ij}, ~B_{ij}, ~ D_{ij} \right\} = \int_{-h/2}^{h/2} \overline{Q}_{ij} \left\{1,~z,~z^2 \right\}~\rmd z
\end{equation}
The thermal stress resultants, $\bn^{\textup{th}}$ and the moment resultants $\bm^{\textup{th}}$ are:

\begin{equation}
\left\{ \bn^{\rm th}, \bm^{\rm th} \right\} = \left\{ \begin{array}{c} N_{xx}^{\textup{th}}, M_{xx}^{\textup{th}} \\ N_{yy}^{\textup{th}}, M_{yy}^{\textup{th}}  \\ N_{xy}^{\textup{th}}, M_{xy}^{\textup{th}}  \end{array} \right\} = \int_{-h/2}^{h/2} \overline{Q}_{ij} \alpha(z,T) \left\{ \begin{array}{c} 1 \\ 1 \\ 0 \end{array} \right\} ~ \Delta T(z)  \left\{1,z \right\} ~ \rmd z
\end{equation}
where the thermal coefficient of expansion $\alpha(z,T)$ is given by \Eref{eqn:thermalcondalpha} and $\Delta T(z) = T(z)-T_o$ is the temperature rise from the reference temperature $T_o$ at which there are no thermal strains. Similarly, the transverse shear force $\mathbf{Q} = \{Q_{xz},Q_{yz}\}$ is related to the transverse shear strains $\bveps_s$ through the following equation:

\begin{equation}
\mathbf{Q} = \mathbf{E} \bveps_s
\end{equation}
 where $\mathbf{E} = E_{ij} = \int_{-h/2}^{h/2} \overline{Q}_{ij} \upsilon_i \upsilon_j~dz;~ (i,j=4,5)$ is the transverse shear stiffness coefficient, $\upsilon_i, \upsilon_j$ is the transverse shear coefficient for non-uniform shear strain distribution through the plate thickness. The stiffness coefficients $\overline{Q}_{ij}$ are defined as:

\begin{eqnarray}
\overline{Q}_{11} = \overline{Q}_{22} = {E(z,T) \over 1-\nu^2}; \hspace{1cm} \overline{Q}_{12} = {\nu E(z,T) \over 1-\nu^2}; \hspace{1cm} \overline{Q}_{16} = \overline{Q}_{26} = 0; \nonumber \\
\overline{Q}_{44} = \overline{Q}_{55} = \overline{Q}_{66} = {E(z,T) \over 2(1+\nu) }; \hspace{1cm} \overline{Q}_{45} = \overline{Q}_{54} = 0.
\end{eqnarray}

\noindent where the modulus of elasticity $E(z,T)$ and Poisson's ratio $\nu$ are given by \Eref{eqn:young}. The strain energy function $U$ is given by:

\begin{equation}
U(\boldsymbol{\delta}) = {1 \over 2} \int_{\Omega} \left\{ \bveps_p^{\textup{T}} \mathbf{A} \bveps_p + \bveps_p^{\textup{T}} \mathbf{B} \bveps_b + 
\bveps_b^{\textup{T}} \mathbf{B} \bveps_p + \bveps_b^{\textup{T}} \mathbf{D} \bveps_b +  \bveps_s^{\textup{T}} \mathbf{E} \bveps_s -  \bveps_p^{\textup{T}} \bn ^{\rm th}- \bveps_b^{\textup{T}} \bm^{\rm th} \right\}~ \rmd\Omega
\label{eqn:potential}
\end{equation}
where $\boldsymbol{\delta} = \{u,v,w,\theta_x,\theta_y\}$ is the vector of the degrees of freedom associated to the displacement field in a finite element discretization. Following the procedure given in~\cite{Rajasekaran1973}, the strain energy function $U$ given in~\Eref{eqn:potential} can be rewritten as:

\begin{equation}
U(\boldsymbol{\delta}) = {1 \over 2}  \boldsymbol{\delta}^{\textup{T}} \mathbf{K}  \boldsymbol{\delta}
\label{eqn:poten}
\end{equation}
where $\mathbf{K}$ is the linear stiffness matrix. The kinetic energy of the plate is given by:

\begin{equation}
T(\boldsymbol{\delta}) = {1 \over 2} \int_{\Omega} \left\{p (\dot{u}_o^2 + \dot{v}_o^2 + \dot{w}_o^2) + I(\dot{\theta}_x^2 + \dot{\theta}_y^2) \right\}~\rmd \Omega
\label{eqn:kinetic}
\end{equation}
where $p = \int_{-h/2}^{h/2} \rho(z)~\rmd z$, $I = \int_{-h/2}^{h/2} z^2 \rho(z)~\rmd z$ and $\rho(z)$ is the mass density that varies through the thickness of the plate. The external work due to the in-plane stress resultants $(N_{xx}^{\textup{th}}, N_{yy}^{\textup{th}}, N_{xy}^{\textup{th}})$ developed in the plate under the thermal load is:

\begin{equation}
\begin{split}
V(\boldsymbol{\delta}) = \int_{\Omega} \left\{ {1 \over 2} \left[ N_{xx}^{\textup{th}} w_{o,x}^2 + N_{yy}^{\textup{th}} w_{o,y}^2 +
2 N_{xy}^{\textup{th}} w_{o,x} w_{o,y}\right] \right. \\
\left. + {h^2 \over 24} \left[ N_{xx}^{\textup{th}} \left( \theta_{x,x}^2 + \theta_{y,x}^2 \right) + N_{yy}^{\textup{th}} \left( \theta_{x,y}^2 + \theta_{y,y}^2 \right) + 2N_{xy}^{\textup{th}} \left( \theta_{x,x} \theta_{x,y} + \theta_{y,x} \theta_{y,y} \right) \right] \right\} ~\rmd \Omega
\end{split}
\label{eqn:potthermal}
\end{equation}
Upon substituting \Erefs{eqn:poten} - (\ref{eqn:potthermal}) in Lagrange's equations of motion, the following governing equation is obtained:

\begin{equation}
\mathbf{M} \ddot{\boldsymbol{\delta}} + (\mathbf{K}+\mathbf{K}_{\rm G}) \boldsymbol{\delta} = \mathbf{0}
\label{eqn:govereqn}
\end{equation}
where $\mathbf{M}$ is the consistent mass matrix. After substituting the characteristic of the time function~\cite{Ganapathi1991} $\ddot{\boldsymbol{\delta}} = -\omega^2 \boldsymbol{\delta}$, the following algebraic equation is obtained:

\begin{equation}
\left( (\mathbf{K}+\mathbf{K}_{\rm G})  - \omega^2 \mathbf{M}\right) \boldsymbol{\delta} = \mathbf{0}
\label{eqn:finaldiscre}
\end{equation}
where $\mathbf{K}$ and $\mathbf{K}_{\rm G}$ are the stiffness matrix and the geometric stiffness matrix due to thermal loads, respectively, $\omega$ is the natural frequency. The plate is subjected to a temperature field. So, the first step in the solution process is to compute the in-plane stress resultants due to the temperature field. These will then be used to compute the stiffness matrix of the system and then the frequencies are computed for the system. \\
